Enabling particle applications for exascale computing platforms

The Exascale Computing Project (ECP) is invested in co-design to assure that key applications are ready for exascale computing. Within ECP, the Co-design Center for Particle Applications (CoPA) is addressing challenges faced by particle-based applications across four sub-motifs: short-range particle-particle interactions (e.g., those which often dominate molecular dynamics (MD) and smoothed particle hydrodynamics (SPH) methods), long-range particle-particle interactions (e.g., electrostatic MD and gravitational N-body), particle-in-cell (PIC) methods, and linear-scaling electronic structure and quantum molecular dynamics (QMD) algorithms. Our crosscutting co-designed technologies fall into two categories: proxy applications (or apps) and libraries. Proxy apps are vehicles used to evaluate the viability of incorporating various types of algorithms, data structures, and architecture-specific optimizations and the associated trade-offs; examples include ExaMiniMD, CabanaMD, CabanaPIC, and ExaSP2. Libraries are modular instantiations that multiple applications can utilize or be built upon; CoPA has developed the Cabana particle library, PROGRESS/BML libraries for QMD, and the SWFFT and fftMPI parallel FFT libraries. Success is measured by identifiable lessons learned that are translated either directly into parent production application codes or into libraries, with demonstrated performance and/or productivity improvement. The libraries and their use in CoPA's ECP application partner codes are also addressed.

==> progress_bml_scheme.tex <==
 \begin{figure}
     \centering
     \begin{tikzpicture}[->,shorten >=1pt,auto,
         block_ct_app/.style ={rectangle, draw=black, 
             very thick, fill=white,
             draw=red!50!black!50,
             top color=white,
             bottom color=magenta!50!black!20,
             text width=24em, text centered,
             minimum height=4em},
         %        
         block_ct_prg/.style ={rectangle, draw=black, 
             very thick, fill=white,
             draw=black,
             top color=white,
             bottom color=blue!50!black!20,
             text width=24em, text centered,
             minimum height=4em},
         %        
         block_ct_bml/.style ={rectangle, draw=black, 
             very thick, fill=white,
             draw=black,
             top color=white,
             bottom color=green!50!black!20,
             text width=24em, text centered,
             minimum height=4em},
         %
         block_ct_nat/.style ={rectangle, draw=black, 
             very thick, fill=white,
             draw=black,
             top color=white,
             bottom color=white!10!black!20,
             text width=24em, text centered,
             font=\scriptsize,
             minimum height=2em},
         %
         block_hf/.style ={rectangle, draw=black, 
             very thick, fill=white,
             draw=black,
             top color=white,
             bottom color=white!10!black!20,
             font=\scriptsize,
             text width=12em, text centered,
             minimum height=2em},        
         %        
         block_hf_cpu/.style ={rectangle, draw=black, 
             very thick, fill=white,
             draw=black,
             top color=white,
             bottom color=yellow!50!black!20, 
             text width=12em, text centered,
             minimum height=4em},        
         %
         block_hf_gpu/.style ={rectangle, draw=black, 
             very thick, fill=white,
             draw=black,
             top color=white,
             bottom color=red!50!black!20, 
             text width=12em, text centered,
             minimum height=4em},        
         %
         main node/.style={circle,draw,font=\Large\bfseries},
         node distance=0em,
         thick,        
         ]
         %
         \node[block_ct_prg] (prg) {\textbf{PROGRESS Solver library - Fortran}};
         \node[block_ct_bml] (bml) [below of=prg,yshift=-4em] {\textbf{Basic Matrix Library (BML) - C, Fortran}
             Matrix formats (dense, ellpack, ellblock, CSR)
             Matrix operations (multiply, add, norm, trace, ...)
         };
         \node[block_hf_cpu] (cpu) [below of=bml,yshift=-4em,xshift=-6em] {\textbf{CPU Only} OpenMP threading};
         \node[block_hf_gpu] (gpu) [right of=cpu, yshift=0em,xshift=12em] {\textbf{CPU + GPU} \hspace{2em} MAGMA, OpenMP offload};
         \node[block_ct_nat] (nat) [below of=bml,yshift=-7em] {\textbf{Native Linear Algebra Libraries} (BLAS, LAPACK) };
         \node[block_hf] (mkl) [below of=nat,yshift=-2em,xshift=-6em] {MKL, OpenBLAS, ESSL,...};
         \node[block_hf] (cub) [right of=mkl,yshift=0em,xshift=12em] {cuBLAS, cuSPARSE};
         %
         \node[block_ct_app] (app) [above of=prg,yshift=4em,xshift=0em] {\textbf{Electronic structure Code}
             \hspace{2em} LATTE, MGMOL, DFTB+
         };
%          \path[->,very thinck]
%          (prg) edge node {} (app);
         
     \end{tikzpicture}
     \caption{Scheme showing the current software stack around PROGRESS and BML libraries. Three-level abstraction model for developing in quantum chemistry. Basic Matrix library
         (BML): Only linear algebra or mathematically related operations are performed. The operations are made
         available through the BML application programming interface. PROGRESS library: This is an archive of
         new capabilities offered as modules that rely entirely on BML. Including graph based parallel e-structure
         solvers and recursive Fermi operators expansion using fast linear scaling algebra. Application code: The
         high-level code that computes a quantum based chemical property. The application code could also be any
         available code such as: LATTE, YAEHMOP, DFTB+, SIESTA, etc. Bottom: Scheme showing a Proxy app
         calling the BML library.}
     \label{fig:stack}
 \end{figure}{}
 

